Close the Loop on the Retrievability Gap

A frozen vision-language encoder now guides image restoration and later indexes what it produced. Over a fixed set of eighteen pansharpening systems on one WorldView-III test set, the fidelity index that ranks them, $Q2^n$ with a reference and HQNR without one, picks the less retrievable of two systems one time in three and one in two; the disagreement lies between the pixel-supervised and the language-conditioned family, and even the best system falls short of the reference, small objects first. We call this the retrievability gap and trace it to the area weighting of position-averaged losses. LEDGER closes the loop around the encoder: it indexes the input into a set of named concepts, generates, re-encodes the output alone with the same frozen encoder, and minimises a set-level soft-Jaccard loss on the coverage of that set, a label-free target available at test time, so that every present concept of a scale receives a gradient share independent of its area. Measured outside the loop by label-grounded probes, held-out retrievers, language-free evaluators, detectors and human raters, LEDGER matches or exceeds the strongest baselines in fidelity on four sensors, raises retrieval by seven to nine points within its vocabulary and two to five outside it, closes two thirds of the reduced-resolution gap to the reference, lifts extraction on raw SpaceNet imagery above the vendor product in each of four cities, and transfers to existing generators as a training-only loss at no inference cost.

==> tables/tab_fiveseeds.tex <==
% generated by figures_src/make_tables.py -- do not edit by hand
\begin{table}[!htbp]
\centering
\caption{The five WorldView-III seeds of \our: reduced-resolution ERGAS / SAM / Q2$^n$, full-resolution HQNR, label-grounded coverage on the annotated full-resolution tiles and concept-query mAP under OpenCLIP.}
\label{tab:fiveseeds}
\scriptsize
\setlength{\tabcolsep}{5pt}
\begin{tabular}{ccccccc}
\toprule
Seed & ERGAS & SAM & Q2$^n$ & HQNR & $\cdino$ & mAP \\
\midrule
0 & 1.955 & 2.675 & 0.931 & 0.966 & 0.85 & 0.506 \\
1 & 1.968 & 2.688 & 0.927 & 0.964 & 0.84 & 0.500 \\
2 & 1.960 & 2.678 & 0.930 & 0.966 & 0.86 & 0.505 \\
3 & 1.966 & 2.683 & 0.928 & 0.965 & 0.85 & 0.502 \\
4 & 1.961 & 2.676 & 0.929 & 0.964 & 0.85 & 0.503 \\
\midrule
mean & 1.962 & 2.680 & 0.929 & 0.965 & 0.85 & 0.503 \\
std & 0.0051 & 0.0054 & 0.0016 & 0.0010 & 0.007 & 0.0024 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/tab_seeds_down.tex <==
% generated by figures_src/make_tables.py -- do not edit by hand
\begin{table}[!htbp]
\centering
\caption{Seed std (three seeds) of the downstream measures of every method of \cref{tab:downstream_rr} on the annotated full-resolution WorldView-III scenes: detection mAP$_{50}$ (points), label-grounded coverage and host concept-query mAP. PAN-only and GSA have no seeds. The differences quoted in the text exceed twice the larger std of the pair in every case.}
\label{tab:seeds_down}
\scriptsize
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lccc}
\toprule
Method & det.\ mAP & $\cdino$ & mAP (host) \\
\midrule
PAN-only & -- & -- & -- \\
GSA & -- & -- & -- \\
CANConv & 0.7 & 0.011 & 0.004 \\
ARConv & 0.6 & 0.009 & 0.004 \\
SGDiff & 0.8 & 0.012 & 0.005 \\
CLIPPan & 0.9 & 0.013 & 0.005 \\
DA-CLIP & 0.9 & 0.012 & 0.005 \\
SeeSR & 1.4 & 0.019 & 0.008 \\
DA-CLIP-style & 0.8 & 0.011 & 0.004 \\
\rowcolor{ourrow}\our & 0.9 & 0.007 & 0.003 \\
\bottomrule
\end{tabular}
\end{table}

